Ludii and XCSP: Playing and Solving Logic Puzzles

Many of the famous single-player games, commonly called puzzles, can be shown to be NP-Complete. Indeed, this class of complexity contains hundreds of puzzles, since people particularly appreciate completing an intractable puzzle, such as Sudoku, but also enjoy the ability to check their solution easily once it's done. For this reason, using constraint programming is naturally suited to solve them. In this paper, we focus on logic puzzles described in the Ludii general game system and we propose using the XCSP formalism in order to solve them with any CSP solver.

==> commands.tex <==
\usepackage[table]{xcolor}
\usepackage{mathrsfs,amssymb,amsmath}
\usepackage{graphicx}
\usepackage{multirow} 
\usepackage{xspace}
\usepackage{booktabs}
\usepackage{enumitem} 
\usepackage{longtable}
\usepackage[htt]{hyphenat} % to allow the cesure of tt text
\usepackage{dirtree}
\usepackage{eurosym}
\usepackage{dirtree}
\definecolor{vlgray}{gray}{0.92}

%
%
%
%\usepackage{tikz}
%\usetikzlibrary{shapes,calc,positioning,automata,arrows,trees}
%\usepackage[tikz]{bclogo}
%\renewcommand\logowidth{15pt}
%\newcommand\bcpen{\includegraphics[width=\logowidth]{figs/bluePen.png}} 
%\newcommand\bcdico{\includegraphics[width=\logowidth]{figs/yellowBook.png}} 
%\newcommand\bcroue{\includegraphics[width=\logowidth]{figs/orangeWheel.png}} 
%\newcommand\bcludii{\includegraphics[width=\logowidth]{figs/ludii-icon-2.pdf}} 
%\newcommand\bcjava{\includegraphics[width=\logowidth]{figs/java-icon-2b.pdf}} 
%\newcommand\bcgrammar{\includegraphics[width=\logowidth]{figs/folder-icon-3.png}} 
%\usepackage[skins,breakable,xparse]{tcolorbox}
%\tikzset{
%  dirtree/.style={
%    grow via three points={one child at (0.8,-0.7) and two children at (0.8,-0.7) and (0.8,-1.45)}, 
%    edge from parent path={($(\tikzparentnode\tikzparentanchor)+(.4cm,0cm)$) |- (\tikzchildnode\tikzchildanchor)}, growth parent anchor=west, parent anchor=south west},
%}

%\usepackage{listingsutf8}

%\lstdefinelanguage{ludii}{
%  keywords={game,metadata,control,rules,keyword,text,time,play,player,equipment,board,square,moves,to,indexOf,empty,end,line,result,index,
%  get,item,component,container,disc,ball,colour,hand,owner,numItems,modify,wheel,hexHex,rect,spokes,aligned,dim,cols,join,cut,remove,cellA,
%  cellB,list,end,start,place,who,count,target,posn,fromTo,or,action,regionFunction,sites,resultType,line,not,occupied,store,length,add
%},
%  basewidth  = {.6em,0.6em},
%  keywordstyle=\color{mblue}\bfseries,
%  ndkeywords={Alternating,Discrete,Real,Mover,Win,Lose,Draw,Tie,Abort,None,Any,All,In,Out,Along,CW,Vert,Horz,F,B,L,R,N,E,S,W,U,D,P1,P2,P3,P4,
%  P5,P6,P7,P8,Opposite,Next,Prev,Odd,Even,Empty,Own,Enemy,Ally,Partner},
%  ndkeywordstyle=\color{dviolet}\bfseries,
%  identifierstyle=\color{black},
%  sensitive=false,
%  comment=[l]{//},
%  morecomment=[s]{<!--}{-->},
%  commentstyle=\color{dred}\ttfamily,
%  stringstyle=\color{dgreen}\ttfamily,
%  morestring=[b]',
%  morestring=[b]",
%  escapechar=@,
%  showstringspaces=false,
%  xleftmargin=1pt,xrightmargin=1pt,
%  breaklines=true,basicstyle=\ttfamily\small,backgroundcolor=\color{colorex},inputencoding=utf8/latin9,texcl
%}
%
%\lstdefinelanguage{syntax}{
%  keywords={game,metadata,control,rules,keyword,text,time,play,player,equipment,board,square,moves,to,indexOf,empty,end,line,result,index,
%  get,item,component,container,disc,ball,colour,hand,owner,numItems,modify,wheel,hexHex,rect,spokes,aligned,dim,cols,join,cut,remove,cellA,
%  cellB,list,end,start,place,who,count,target,posn,fromTo,or,action,regionFunction,sites,resultType,line,not,occupied,store,where,what,class,
%  arg,subClass,terminal,add,roleType,knight,cross,bishop,king,queen,pawn,rook,piece,card,die,letter,number,tile,chess,timeType,basis,label,
%  rows,players,name,and,dirn,dirnType,length,sitesFrom,sitesTo,functions,cont,site,role,num,types,cell
%},
%  keywordstyle=\color{dblue}\slshape,ndkeywords={String,int,boolean,string,ints,booleans},
%  ndkeywordstyle=\color{dviolet}\bfseries,
%  basewidth  = {.5em,0.5em},
%  escapechar=@,
%  xleftmargin=1pt,xrightmargin=1pt,
%  breaklines=true,basicstyle=\ttfamily\linespread{1.0}\small,backgroundcolor=\color{colorsy},inputencoding=utf8/latin9,texcl
%}
%
%\definecolor{javared}{rgb}{0.6,0,0} % for strings
%\definecolor{javagreen}{rgb}{0.25,0.5,0.35} % comments
%\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
%\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc
 
%\lstset{language=Java,
%basicstyle=\small,
%keywordstyle=\color{javapurple}\bfseries,
%stringstyle=\color{javared},
%commentstyle=\color{javagreen},
%morecomment=[s][\color{javadocblue}]{/**}{*/},
%tabsize=4,
%showspaces=false,
%showstringspaces=false}
%
%\newcommand{\core}[1]{ 
%  \medskip \begin{tcolorbox}[
%    enhanced,breakable,
%    boxsep=0pt,top=0pt,bottom=0pt,left=6mm,right=1mm,
%    toprule=0.1mm,leftrule=0.1mm,rightrule=0.25mm,bottomrule=0.25mm,shadow={0.2mm}{-0.2mm}{0mm}{dgray},
%    overlay unbroken and first={\node (logo) at ([xshift=4mm,yshift=-5mm]frame.north west) {#1}; %\draw[black,line width=1.5pt] (logo) -- ([xshift=4mm,yshift=1.5mm]frame.south west);  
%    },
%    colframe=dgray,titlerule=-0.2mm,toptitle=3mm,coltitle=black,fonttitle=\bfseries,
%    lines before break=6, pad at break*=10pt
%}
%\newcounter{cntJa}
%\newcounter{cntEx}
%\newcounter{cntSy}
%
%%\def\bw{1}
%\ifx\bw\undefined
%  \lstnewenvironment{java}{\lstset{language=java}}{}
%  \lstnewenvironment{ludii}{\lstset{language=ludii}}{} 
%  \lstnewenvironment{syntax}{\lstset{language=syntax}}{} 
%    \newenvironment{boxja}
%    {\stepcounter{cntJa} \core{\bcjava} ,colback=colorja,title style={color=colorja},title=~ Java \thecntJa]}
%    {\end{tcolorbox}} %{\vspace{-0.1cm}\end{tcolorbox} ~ \vspace{-0.2cm}}
%  \newenvironment{boxex}
%    {\stepcounter{cntEx} \core{\bcludii} ,colback=colorex,title style={color=colorex},title=~ Ludeme \thecntEx]}
%    {\end{tcolorbox}} %{\vspace{-0.1cm}\end{tcolorbox} ~ \vspace{-0.2cm}}
%  \newenvironment{boxsy}
%    {\stepcounter{cntSy} \core{\bcgrammar} ,colback=colorsy,title style={color=colorsy},title=~ Grammar \thecntSy]}
%    {\end{tcolorbox}} %{\vspace{-0.1cm}\end{tcolorbox} ~ \vspace{-0.2cm}}
%
%
%\newtheorem{definition}{Definition}
%\newtheorem{remark}{Remark}
%
%\definecolor{v2lgray}{gray}{0.85}
%\definecolor{dgray}{rgb}{0.4,0.4,0.4}
%\definecolor{dblue}{RGB}{0,0,99}
%\definecolor{dred}{RGB}{150,6,54}
%\definecolor{dgreen}{RGB}{47,135,7}
%\definecolor{dviolet}{RGB}{102,0,153}
%\definecolor{mblue}{RGB}{0,0,180}
%\definecolor{colorja}{RGB}{255,248,220}
%\definecolor{colorex}{HTML}{DFEFFF}  %{FFE3BE}
%\definecolor{colorsy}{HTML}{F2F2F2}
%\definecolor{grey1}{rgb}{0.9,0.9,0.9}

\def\AI{{\rm {\sc AI}}\xspace}
\def\MCTS{{\rm {\sc MCTS}}\xspace}
\def\LUDII{{\rm {\sc Ludii}}\xspace}
\def\GGPBASE{{\rm {\sc GGP-BASE}}\xspace}
\def\GGP{{\rm {\sc GGP}}\xspace}
\def\GDL{{\rm {\sc GDL}}\xspace}
\def\GDLII{{\rm {\sc GDL-II}}\xspace}
\def\GDLIII{{\rm {\sc GDL-III}}\xspace}
\def\DLP{{\rm {\sc DLP}}\xspace}
\def\RBG{{\rm {\sc RBG}}\xspace}
\def\BGG{{\rm {\sc BGG}}\xspace}
\def\ZRF{{\rm {\sc ZRF}}\xspace}
\def\AAAI{{\rm {\sc AAAI}}\xspace}

%\newcommand{\bnf}[1]{\textsl{\color{dblue}{#1}}}
%\newcommand{\bnfX}[1]{\texttt{<}\bnf{#1}\texttt{.../>}}
%\newcommand{\norX}[1]{\texttt{<#1.../>}}

\newcommand{\todoguys}[1]{\fbox{{\footnotesize\textcolor{red}{{\bf TODO : #1}}}}}
\definecolor{grey}{rgb}{0.75,0.75,0.75}


\newtheorem{definition}{Definition}
\newtheorem{example}{Example}


\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{proof}{Proof}
